ReplaceAnything3D:Text-Guided 3D Scene Editing with Compositional Neural Radiance Fields

We introduce ReplaceAnything3D model (RAM3D), a novel text-guided 3D scene editing method that enables the replacement of specific objects within a scene. Given multi-view images of a scene, a text prompt describing the object to replace, and a text prompt describing the new object, our Erase-and-Replace approach can effectively swap objects in the scene with newly generated content while maintaining 3D consistency across multiple viewpoints. We demonstrate the versatility of ReplaceAnything3D by applying it to various realistic 3D scenes, showcasing results of modified foreground objects that are well-integrated with the rest of the scene without affecting its overall integrity.

==> Figures/Compare_IN2N.tex <==
\begin{figure*}
\centering
     \includegraphics[width=0.8\linewidth]{Figures/pdf/Compare_IN2N.pdf}
    \caption{Comparison with Instruct-NeRF2NeRF.}
    \label{fig:compare_IN2N}
\end{figure*}

==> Figures/Compare_ReferenceGuided.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]
    {Figures/pdf/Adding_ReferenceGuided.pdf} 
    \caption{Qualitative comparison with method by \citet{mirzaei_reference-guided_2023} for object replacement. Figure adapted from the original paper by \citet{mirzaei_reference-guided_2023}.}
    \label{fig:compare_RefGuided}
\end{figure}


==> Figures/Removal_comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/pdf/Removal.pdf}
    \caption{Qualitative comparison for object removal and background inpainting task. Although object removal is not the main focus of $\name$, our method can achieve competitive results with state-of-the-art methods.}
    \label{fig:removal}
\end{figure}

==> Figures/adding_qualitative.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/pdf/adding_qualitative_results.pdf}
    \caption{Given users' defined masks, $\name$ can also add completely new objects that blend in with the rest of the scene.}
    \label{fig:object_adding}
\end{figure}

==> Figures/blendedNeRF.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]
    {Figures/pdf/Adding_blendNeRF.pdf} 
    \caption{Qualitative comparison with Blended-NeRF for object replacement. Our method generates results with higher quality and capture more realistic lighting and details.}
    \label{fig:blendedNeRF}
\end{figure}


==> Figures/corgis_ablation.tex <==
% \usepackage[demo]{graphicx}
% \usepackage{subfig}
\begin{figure}%
    %\centering
    %   \subfloat[\centering Our Monolithic Model]{{\includegraphics[width=\columnwidth]{Figures/pdf/corgi_monolithic.pdf} }}%
    %\qquad
    %    \subfloat[\centering Our Composited Model, without random background augmentation]{{\includegraphics[width=\columnwidth]{Figures/pdf/corgi_no_augmentation.pdf} }}%
    %     \qquad   
    %\subfloat[\centering Our Full Composited Model]{{\includegraphics[width=\columnwidth]{Figures/pdf/corgi_full.pdf} }}%
    \centering
    \includegraphics[width=\columnwidth]{Figures/pdf/corgi_ablation_revise.pdf}
    \caption{Ablation results for 3 RAM variants, on the statue scene, with Corgi prompt.
    RGB samples are shown with accumulated NeRF transmittence (alpha map) in the top-left corner.
    Bubble rendering region is shown as a dotted blue line.
    In a), we show the result of training
    a monolithic model which represents the foreground object and inpainted background
    in a single 3D implicit. In b), we instead use a composited model, without random background augmentation. In c), we show the results of our full model}%
    \label{fig:ablation}%
\end{figure}

==> Figures/plinth_ablation.tex <==
% \usepackage[demo]{graphicx}
% \usepackage{subfig}
\begin{figure}%
    %\centering
    %   \subfloat[\centering Our Monolithic Model]{{\includegraphics[width=\columnwidth]{Figures/pdf/corgi_monolithic.pdf} }}%
    %\qquad
    %    \subfloat[\centering Our Composited Model, without random background augmentation]{{\includegraphics[width=\columnwidth]{Figures/pdf/corgi_no_augmentation.pdf} }}%
    %     \qquad   
    %\subfloat[\centering Our Full Composited Model]{{\includegraphics[width=\columnwidth]{Figures/pdf/corgi_full.pdf} }}%
    \centering
    \includegraphics[width=0.8\columnwidth]{Figures/pdf/plinth_ablation.pdf}
    \caption{Ablation showing the importance of halo-region supervision to our approach.
    We show results for 2 RAMs trained on the Statue scene, with object removal prompt.
    In a), we show the result of training without any loss supervision on the halo region, surrounding the
    inpainting mask. The bubble-NeRF model collapses to a hazy cloud. In b), we show that the same model trained with
    halo loss supervision added back in achieves a successful inpainting of the background scene.}%
    \label{fig:plinth_ablation}%
\end{figure}
